Symbolic Loop Compilation for Tightly Coupled Processor Arrays

Loop compilation for Tightly Coupled Processor Arrays (TCPAs), a class of massively parallel loop accelerators, entails solving NP-hard problems, yet depends on the loop bounds and number of available processing elements (PEs), parameters known only at runtime because of dynamic resource management and input sizes. Therefore, this article proposes a two-phase approach called symbolic loop compilation: At compile time, the necessary NP-complete problems are solved and the solutions compiled into a space-efficient symbolic configuration. At runtime, a concrete configuration is generated from the symbolic configuration according to the parameters values. We show that the latter phase, called instantiation, runs in polynomial time with its most complex step, program instantiation, not depending on the number of PEs. As validation, we performed symbolic loop compilation on real-world loops and measured time and space requirements. Our experiments confirm that a symbolic configuration is space-efficient and suited for systems with little memory -- often, a symbolic configuration is smaller than a single concrete configuration -- and that program instantiation scales well with the number of PEs -- for example, when instantiating a symbolic configuration of a matrix-matrix multiplication, the execution time is similar for $4\times 4$ and $32\times 32$ PEs.

==> figures/tikz/cfg-2.tex <==
\begin{tikzpicture}[
  cfg node/.style={draw,inner sep=0pt,minimum size=1cm,font=\small},
  cfg node all/.style={
    cfg node,
  },
  cfg edge/.style={->,>=latex},
  node distance=0cm and 1.5cm,
]
  \node[cfg node all,draw=contrastB!70!black,fill=contrastB!50] (pb0) {PB0};
\end{tikzpicture}




==> head/tikz.tex <==
\makeatletter

\pgfkeys{/pgf/.cd,
  rectangle corner radius north west/.initial=10pt,
  rectangle corner radius north east/.initial=10pt,
  rectangle corner radius south west/.initial=10pt,
  rectangle corner radius south east/.initial=10pt
}
\newif\ifpgf@rectanglewrc@donecorner@
\def\pgf@rectanglewithroundedcorners@docorner#1#2#3#4#5{%
  \edef\pgf@marshal{%
    \noexpand\pgfintersectionofpaths
      {%
        \noexpand\pgfpathmoveto{\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
        \noexpand\pgfpathlineto{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
      }%
      {%
        \noexpand\pgfpathmoveto{\noexpand\pgfpointadd
          {\noexpand\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}%
          {\noexpand\pgfpoint{#1}{#2}}}%
        \noexpand\pgfpatharc{#3}{#4}{#5}%
      }%
    }%
  \pgf@process{\pgf@marshal\pgfpointintersectionsolution{1}}%
  \pgf@process{\pgftransforminvert\pgfpointtransformed{}}%
  \pgf@rectanglewrc@donecorner@true
}
\pgfdeclareshape{rectangle with rounded corners}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}

  \savedmacro\cornerradiusnw{%
    \edef\cornerradiusnw{\pgfkeysvalueof{/pgf/rectangle corner radius north west}}%
  }
  \savedmacro\cornerradiusne{%
    \edef\cornerradiusne{\pgfkeysvalueof{/pgf/rectangle corner radius north east}}%
  }
  \savedmacro\cornerradiussw{%
    \edef\cornerradiussw{\pgfkeysvalueof{/pgf/rectangle corner radius south west}}%
  }
  \savedmacro\cornerradiusse{%
    \edef\cornerradiusse{\pgfkeysvalueof{/pgf/rectangle corner radius south east}}%
  }

  \backgroundpath{%
    \northeast\advance\pgf@y-\cornerradiusne\relax
    \pgfpathmoveto{}%
    \pgfpatharc{0}{90}{\cornerradiusne}%
    \northeast\pgf@ya=\pgf@y\southwest\advance\pgf@x\cornerradiusnw\relax\pgf@y=\pgf@ya
    \pgfpathlineto{}%
    \pgfpatharc{90}{180}{\cornerradiusnw}%
    \southwest\advance\pgf@y\cornerradiussw\relax
    \pgfpathlineto{}%
    \pgfpatharc{180}{270}{\cornerradiussw}%
    \northeast\pgf@xa=\pgf@x\advance\pgf@xa-\cornerradiusse\southwest\pgf@x=\pgf@xa
    \pgfpathlineto{}%
    \pgfpatharc{270}{360}{\cornerradiusse}%
    \northeast\advance\pgf@y-\cornerradiusne\relax
    \pgfpathlineto{}%
    \pgfpathclose
  }

  \anchor{before north east}{\northeast\advance\pgf@y-\cornerradiusne}
  \anchor{after north east}{\northeast\advance\pgf@x-\cornerradiusne}
  \anchor{before north west}{\southwest\pgf@xa=\pgf@x\advance\pgf@xa\cornerradiusnw
    \northeast\pgf@x=\pgf@xa}
  \anchor{after north west}{\northeast\pgf@ya=\pgf@y\advance\pgf@ya-\cornerradiusnw
    \southwest\pgf@y=\pgf@ya}
  \anchor{before south west}{\southwest\advance\pgf@y\cornerradiussw}
  \anchor{after south west}{\southwest\advance\pgf@x\cornerradiussw}
  \anchor{before south east}{\northeast\pgf@xa=\pgf@x\advance\pgf@xa-\cornerradiusse
    \southwest\pgf@x=\pgf@xa}
  \anchor{after south east}{\southwest\pgf@ya=\pgf@y\advance\pgf@ya\cornerradiusse
    \northeast\pgf@y=\pgf@ya}

  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
    \pgfextract@process\borderpoint{}%
    %
    \pgf@rectanglewrc@donecorner@false
    %
    % do southwest corner
    \southwest\pgf@xc=\pgf@x\pgf@yc=\pgf@y
    \advance\pgf@xc\cornerradiussw\relax\advance\pgf@yc\cornerradiussw\relax
    \borderpoint
    \ifdim\pgf@x<\pgf@xc\relax\ifdim\pgf@y<\pgf@yc\relax
      \pgf@rectanglewithroundedcorners@docorner{-\cornerradiussw}{0pt}{180}{270}{\cornerradiussw}%
    \fi\fi
    %
    % do southeast corner
    \ifpgf@rectanglewrc@donecorner@\else
      \southwest\pgf@yc=\pgf@y\relax\northeast\pgf@xc=\pgf@x\relax
      \advance\pgf@xc-\cornerradiusse\relax\advance\pgf@yc\cornerradiusse\relax
      \borderpoint
      \ifdim\pgf@x>\pgf@xc\relax\ifdim\pgf@y<\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{0pt}{-\cornerradiusse}{270}{360}{\cornerradiusse}%
      \fi\fi
    \fi
    %
    % do northeast corner
    \ifpgf@rectanglewrc@donecorner@\else
      \northeast\pgf@xc=\pgf@x\relax\pgf@yc=\pgf@y\relax
      \advance\pgf@xc-\cornerradiusne\relax\advance\pgf@yc-\cornerradiusne\relax
      \borderpoint
      \ifdim\pgf@x>\pgf@xc\relax\ifdim\pgf@y>\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{\cornerradiusne}{0pt}{0}{90}{\cornerradiusne}%
      \fi\fi
    \fi
    %
    % do northwest corner
    \ifpgf@rectanglewrc@donecorner@\else
      \northeast\pgf@yc=\pgf@y\relax\southwest\pgf@xc=\pgf@x\relax
      \advance\pgf@xc\cornerradiusnw\relax\advance\pgf@yc-\cornerradiusnw\relax
      \borderpoint
      \ifdim\pgf@x<\pgf@xc\relax\ifdim\pgf@y>\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{0pt}{\cornerradiusnw}{90}{180}{\cornerradiusnw}%
      \fi\fi
    \fi
  }
}

\makeatother

\tikzset{%
  iteration/.style={
    rectangle with rounded corners,
    rectangle corner radius north west = 0.125cm,
    rectangle corner radius south west = 0.125cm,
    rectangle corner radius north east = 0.125cm,
    rectangle corner radius south east = 0.125cm,
    draw,
    inner sep=0pt,
    minimum size=0.25cm
  },%
  iteration none/.style={
    iteration,
  },%
  iteration left/.style={
    iteration,
    rectangle corner radius north west = 0pt,
    rectangle corner radius south west = 0pt,
  },%
  iteration top/.style={
    iteration, 
    rectangle corner radius north west = 0pt,
    rectangle corner radius north east = 0pt,
  },%
  iteration bottom/.style={
    iteration, 
    rectangle corner radius south west = 0pt,
    rectangle corner radius south east = 0pt,
  },%
  iteration right/.style={
    iteration, 
    rectangle corner radius north east = 0pt,
    rectangle corner radius south east = 0pt,
  },%
  iteration bottom right/.style={
    iteration, 
    rectangle corner radius south east = 0pt,
    rectangle corner radius north east = 0pt,
    rectangle corner radius south west = 0pt,
  },%
  iteration bottom left/.style={
    iteration, 
    rectangle corner radius south west = 0pt,
    rectangle corner radius north west = 0pt,
    rectangle corner radius south east = 0pt,
  },%
  iteration all/.style={
    iteration, 
    rectangle corner radius north east = 0pt,
    rectangle corner radius south west = 0pt,
    rectangle corner radius north west = 0pt,
    rectangle corner radius south east = 0pt,
  },%
  iteration top right/.style={
    iteration, 
    rectangle corner radius south east = 0pt,
    rectangle corner radius north east = 0pt,
    rectangle corner radius north west = 0pt,
  },%
  iteration top left/.style={
    iteration, 
    rectangle corner radius south west = 0pt,
    rectangle corner radius north west = 0pt,
    rectangle corner radius north east = 0pt,
  },%
  dependence/.style={
    ->, >=latex, gray
  }
}

%\definecolor{contrastA}{HTML}{f1a340}
%\definecolor{contrastB}{HTML}{998ec3}
%\definecolor{contrastC}{HTML}{d0d000}
%\definecolor{contrastD}{HTML}{8dd3c7}
\definecolor{contrastA}{HTML}{8dd3c7}
\definecolor{contrastB}{HTML}{ffffb3}
\definecolor{contrastC}{HTML}{bebada}
\definecolor{contrastD}{HTML}{fb8072}

\newif\ifuseprotrusion
%\useprotrusiontrue

\ifuseprotrusion
\newcommand{\iteration}[4]{%
\node[iteration,draw=#4!70!black,fill=#4!50] at (i-#1-#2) {};
}
\newcommand{\protrusion}[4]{%
\fill[#3!70!black] (i-#1-#2.#4) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
}
\newcommand{\Irightbottomleft}[3]{%
\fill[#3!70!black] (i-#1-#2.west) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.south) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.east) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Ilefttopright}[3]{%
\fill[#3!70!black] (i-#1-#2.west) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.north) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.east) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Ibottomright}[3]{%
\fill[#3!70!black] (i-#1-#2.south) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.east) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Ibottomleft}[3]{%
\fill[#3!70!black] (i-#1-#2.south) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.west) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Itopright}[3]{%
\fill[#3!70!black] (i-#1-#2.north) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.east) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Itopleft}[3]{%
\fill[#3!70!black] (i-#1-#2.north) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.west) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Itoprightbottom}[3]{%
\fill[#3!70!black] (i-#1-#2.south) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.north) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.east) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Itopleftbottom}[3]{%
\fill[#3!70!black] (i-#1-#2.south) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.north) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\fill[#3!70!black] (i-#1-#2.west) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Itop}[3]{%
\protrusion{#1}{#2}{#3}{north}
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Ibottom}[3]{%
\protrusion{#1}{#2}{#3}{south}
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Ileft}[3]{%
\fill[#3!70!black] (i-#1-#2.west) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Iright}[3]{%
\fill[#3!70!black] (i-#1-#2.east) ++(-0.0625,-0.0625) rectangle +(0.125,0.125);
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Iall}[3]{%
\protrusion{#1}{#2}{#3}{north}
\protrusion{#1}{#2}{#3}{south}
\protrusion{#1}{#2}{#3}{west}
\protrusion{#1}{#2}{#3}{east}
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}
\newcommand{\Inone}[3]{%
\node[iteration,draw=#3!70!black,fill=#3!50] at (i-#1-#2) {};
}

\else

\newcommand{\iteration}[4]{%
\node[iteration #3,draw=#4!70!black,fill=#4!50] at (i-#1-#2) {};
}
\newcommand{\Irightbottomleft}[3]{%
\iteration{#1}{#2}{all}{#3}
}
\newcommand{\Ilefttopright}[3]{%
\iteration{#1}{#2}{all}{#3}
}
\newcommand{\Ibottomright}[3]{%
\iteration{#1}{#2}{bottom right}{#3}
}
\newcommand{\Ibottomleft}[3]{%
\iteration{#1}{#2}{bottom left}{#3}
}
\newcommand{\Itopright}[3]{%
\iteration{#1}{#2}{top right}{#3}
}
\newcommand{\Itopleft}[3]{%
\iteration{#1}{#2}{top left}{#3}
}
\newcommand{\Itoprightbottom}[3]{%
\iteration{#1}{#2}{all}{#3}
}
\newcommand{\Itopleftbottom}[3]{%
\iteration{#1}{#2}{all}{#3}
}
\newcommand{\Itop}[3]{%
\iteration{#1}{#2}{top}{#3}
}
\newcommand{\Ibottom}[3]{%
\iteration{#1}{#2}{bottom}{#3}
}
\newcommand{\Ileft}[3]{%
\iteration{#1}{#2}{left}{#3}
}
\newcommand{\Iright}[3]{%
\iteration{#1}{#2}{right}{#3}
}
\newcommand{\Iall}[3]{%
\iteration{#1}{#2}{all}{#3}
}
\newcommand{\Inone}[3]{%
\iteration{#1}{#2}{none}{#3}
}
\fi

\newcommand{\iterations}[2]{%
\foreach \y in {1,...,#1} {%
  \foreach \x in {1,...,#2} {%
    \node[iteration,draw=none,fill=none] (i-\y-\x) at ($0.625*(\x,-\y)$) {};}}}

\newcommand{\dependences}{%
\ifshowdependences
  \foreach \i in {1,2,3,4,5} {
    \pgfmathtruncatemacro\ni{\i+1}
    \foreach \j in {1,2,3,4,5,6} {
      \path[->,>=latex,gray] (i-\i-\j) edge (i-\ni-\j);
      \path[->,>=latex,gray] (i-\j-\i) edge (i-\j-\ni);
    }
  }
\fi}

\newif\ifshowdependences
\showdependencestrue



==> sections/periphery.tex <==
\section{Generation of periphery configuration}
\label{sec:periphery-configuration}

Of course, the configuration of a \ac{TCPA} not only consists of \ac{PE} programs, but also of a configuration for the periphery: interconnect network, buffers, and a global controller.

\subsection{Interconnect configuration}

Propagation channel allocation at compile time.
Routing from input/output ports to buffers at runtime.

\subsection{Buffers}

Address generator configuration at runtime from $Q, d$, and $\mathcal I$.

\subsection{Global controller}

Generate program blocks from polyhedral syntax tree at runtime.


==> sections/table-buffer-instantiation.tex <==
\begin{tikzpicture}
  \draw[thick, <->, >=latex]
    (0, 0) -- ++(down:2) -- ++(right:8) node[right] {\acp{PE}};

  \node[left, align=right] at (-1, -1) {Normalized\\Runtime\\(\textbf{I/O Instantiation})};

  \draw
    (0.125, -0.5) -- ++(left:0.25) node[left] {100}
    (0.125, -1.0) -- ++(left:0.25) node[left] {10}
    (0.125, -1.5) -- ++(left:0.25) node[left] {1};

  \draw
    (1, -1.875) -- ++(down:0.25) node[below] {1}
    (3.4, -1.875) -- ++(down:0.25) node[below] {16}
    (4, -1.875) -- ++(down:0.25) node[below] {32}
    (4.6, -1.875) -- ++(down:0.25) node[below] {64}
    (7, -1.875) -- ++(down:0.25) node[below] {1024}
    ;

  \node[inner sep=0pt, minimum size=0.1cm, circle, draw, fill=black] (measurement-1) at (1, -1.5) {};
  \node[inner sep=0pt, minimum size=0.1cm, circle, draw, fill=black] at (3.4, -1) {};
  \node[inner sep=0pt, minimum size=0.1cm, circle, draw, fill=black] at (4, -0.89) {};
  \node[inner sep=0pt, minimum size=0.1cm, circle, draw, fill=black] at (4.6, -0.7) {};
  \node[inner sep=0pt, minimum size=0.1cm, circle, draw, fill=black] (measurement-1024) at (7, -0.05) {};

  \draw[densely dashed, shorten >=-0.25cm, shorten <=-0.25cm] (measurement-1) -- (measurement-1024);

\end{tikzpicture}
